ProTuner: Tuning Programs with Monte Carlo Tree Search

We explore applying the Monte Carlo Tree Search (MCTS) algorithm in a notoriously difficult task: tuning programs for high-performance deep learning and image processing. We build our framework on top of Halide and show that MCTS can outperform the state-of-the-art beam-search algorithm. Unlike beam search, which is guided by greedy intermediate performance comparisons between partial and less meaningful schedules, MCTS compares complete schedules and looks ahead before making any intermediate scheduling decision. We further explore modifications to the standard MCTS algorithm as well as combining real execution time measurements with the cost model. Our results show that MCTS can outperform beam search on a suite of 16 real benchmarks.

==> dse.tex <==
\section{Design Space Exploration}
One of the most challenging tasks of designing the MCTS was finding the right configurations, which includes hyperparamter tuning, reward engineering, and finding the right trade-off between greediness and randomness. Our main objective was to find optimal schedules as fast as possible. This is challenging because while MCTS has optimality guarantees it often runs for a prolonged period of time, which can make our approach less attractive.

We start with the UCB equation:
\begin{equation}
    UCB = \bar{X_j} + C_p\sqrt{\frac{2ln(n)}{n_j}}
\end{equation}

The reward can be defined as the negative execution-time. But in that case the MCTS will rarely explore because of the high value and range of the execution-times. Therefore, we set the reward to $\frac{1}{execution_time}$. In that case our reward is bounded between 0 and 1. Kocsis \textit{et al.}~\cite{kocsis2006improved} has shown that $C_p = \sqrt(2)$ works well with rewards in range $[0,1]$ as it satisfies the Hoeffding inequality. Increasing $C_p$ will add more exploration, and decreasing it will reduce exploration. In our case, the cost model predicts execution times that results in very small rewards, and hence the exploitation phase starts very late. This might be useful in very large benchmarks, but since we want to limit the runtime of the MCTS, we chose $C_p$ to be equal to the average reward of the node. This puts $C_p$ in the range of the reward values and encourages earlier exploitation without compromising exploration.



